A Novel Unified Architecture for Low-Shot Counting by Detection and Segmentation

Low-shot object counters estimate the number of objects in an image using few or no annotated exemplars. Objects are localized by matching them to prototypes, which are constructed by unsupervised image-wide object appearance aggregation. Due to potentially diverse object appearances, the existing approaches often lead to overgeneralization and false positive detections. Furthermore, the best-performing methods train object localization by a surrogate loss, that predicts a unit Gaussian at each object center. This loss is sensitive to annotation error, hyperparameters and does not directly optimize the detection task, leading to suboptimal counts. We introduce GeCo, a novel low-shot counter that achieves accurate object detection, segmentation, and count estimation in a unified architecture. GeCo robustly generalizes the prototypes across objects appearances through a novel dense object query formulation. In addition, a novel counting loss is proposed, that directly optimizes the detection task and avoids the issues of the standard surrogate loss. GeCo surpasses the leading few-shot detection-based counters by $\sim$25\% in the total count MAE, achieves superior detection accuracy and sets a new solid state-of-the-art result across all low-shot counting setups.

==> cutout_text.tex <==
% The primary objective of the novel training approach is to devise a loss that enables the method to authomously select the optimal location for predicting the object bounding box, rather than constraining it to predict it from the center of the object~\cite{dave,tian2019fcos}. 
% Furthermore, training the method to align with noisy point annotations, which approximate object centers, and penalizing models for deviations from the center, even if they remain within the object, is undesirable. 
% State-of-the-art methods show that adjusting the sigma of the Gaussian based on the size of exemplars improves performance. Consequently, autonomously selecting the best sigma and even accommodating arbitrary distributions for different objects is needed.
% Furthermore, training for center prediction is an auxiliary, surrogate task, not directly optimized for detection.
% Based on outlined challenges, we propose a training setup that allows the method to select the optimal location for bounding box prediction as follows. 

% A $3\times 3$ non-maximum suppression (NMS) is first applied on a 2D objectness scores $\mathbf{y}^{\mathrm{C}}$ to get a set of 2D spatial locations $X = \{ (x_i, y_i) \}_{i=1:N^{\mathrm{P}}}$.
% Note that only locations where $\mathbf{y}^{\mathrm{C}}_i$ is larger than the median value in $\mathbf{y}^{\mathrm{C}}_i$ are kept to filter out obvious poor detections while keeping high recall.  
% A set of predicted bounding boxes $\boldsymbol{B}^{P}$ is obtained by reading out the predictions from $\mathbf{y}^{\mathrm{BB}}_i$ on spatial locations $i \in X$. 
